DeRS: Towards Extremely Efficient Upcycled Mixture-of-Experts Models

Upcycled Mixture-of-Experts (MoE) models have shown great potential in various tasks by converting the original Feed-Forward Network (FFN) layers in pre-trained dense models into MoE layers. However, these models still suffer from significant parameter inefficiency due to the introduction of multiple experts. In this work, we propose a novel DeRS (Decompose, Replace, and Synthesis) paradigm to overcome this shortcoming, which is motivated by our observations about the unique redundancy mechanisms of upcycled MoE experts. Specifically, DeRS decomposes the experts into one expert-shared base weight and multiple expert-specific delta weights, and subsequently represents these delta weights in lightweight forms. Our proposed DeRS paradigm can be applied to enhance parameter efficiency in two different scenarios, including: 1) DeRS Compression for inference stage, using sparsification or quantization to compress vanilla upcycled MoE models; and 2) DeRS Upcycling for training stage, employing lightweight sparse or low-rank matrixes to efficiently upcycle dense models into MoE models. Extensive experiments across three different tasks show that the proposed methods can achieve extreme parameter efficiency while maintaining the performance for both training and compression of upcycled MoE models.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/ablation_DeRS_LD.tex <==
\begin{table}[!t]
\caption{Ablation on the effect}
  \label{tab:ablation_DeRS_LD}
  \resizebox{1.0\linewidth}{!}{
  \renewcommand\arraystretch{1.35}
  \centering
  \begin{tabular}{c|c|cc|c}
    \toprule
     \textbf{\begin{tabular}[c]{@{}c@{}}DeRS-LD\\ Rank\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Added\\ Params.\end{tabular}} & \textbf{HumanEval (+)} & \textbf{MBPP (+)} & \textbf{Overall} \\
    \midrule
    1  & \textcolor{gray}{0.81B}+2.57M & 64.6 (61.6) & 63.4 (51.1) & 60.2 \\
    4  & \textcolor{gray}{0.81B}+9.09M & 65.9 (62.8) & 62.9 (51.9) & 60.9 \\ 
    16 & \textcolor{gray}{0.81B}+35.2M & 65.9 (62.2) & 63.2 (51.4) & 60.7 \\ 
    64 & \textcolor{gray}{0.81B}+140M & 63.4 (59.1) & 62.7 (50.9) & 59.0 \\ 
    \bottomrule
  \end{tabular}}
\end{table}

==> tables/ablation_DeRS_SM.tex <==
\begin{table}[!t]
\caption{\textbf{}}
  \label{tab:ablation_DeRS_SM}
  \resizebox{1.0\linewidth}{!}{
  \renewcommand\arraystretch{1.35}
  \centering
  \begin{tabular}{c|c|cc|c}
    \toprule
     \textbf{\begin{tabular}[c]{@{}c@{}}DeRS-SM\\ Ratio\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Added\\ Params.\end{tabular}} & \textbf{HumanEval (+)} & \textbf{MBPP (+)} & \textbf{Overall} \\
    \midrule
    0.9999 & \textcolor{gray}{0.81B}+0.72M & 62.8 (60.4) & 63.7 (51.6) & 59.6 \\
    0.999  & \textcolor{gray}{0.81B}+3.64M & 64.0 (60.4) & 63.4 (51.6) & 59.9 \\ 
    0.99   & \textcolor{gray}{0.81B}+32.9M & 64.6 (61.6) & 62.7 (51.4) & 60.1 \\ 
    0.9    & \textcolor{gray}{0.81B}+325M & 66.5 (62.8) & 63.4 (51.4) & 61.0 \\ 
    \bottomrule
  \end{tabular}}
\end{table}
